STAND-Guard: A Small Task-Adaptive Content Moderation Model

Content moderation, the process of reviewing and monitoring the safety of generated content, is important for development of welcoming online platforms and responsible large language models. Content moderation contains various tasks, each with its unique requirements tailored to specific scenarios. Therefore, it is crucial to develop a model that can be easily adapted to novel or customized content moderation tasks accurately without extensive model tuning. This paper presents STAND-GUARD, a Small Task-Adaptive coNtent moDeration model. The basic motivation is: by performing instruct tuning on various content moderation tasks, we can unleash the power of small language models (SLMs) on unseen (out-of-distribution) content moderation tasks. We also carefully study the effects of training tasks and model size on the efficacy of cross-task fine-tuning mechanism. Experiments demonstrate STAND-Guard is comparable to GPT-3.5-Turbo across over 40 public datasets, as well as proprietary datasets derived from real-world business scenarios. Remarkably, STAND-Guard achieved nearly equivalent results to GPT-4-Turbo on unseen English binary classification tasks

==> src/sec7-limitations.tex <==
\section{Limitations}
\vspace{-0.15cm}
The training data, derived from publicly available content moderation datasets, lacks the requisite diversity to encompass a broad spectrum of languages and the full gamut of binary and multi-class classification tasks. Additionally, the foundational model, Mistral-7B, does not come with assured multi-lingual capabilities. These constraints impede the comprehensive assessment of knowledge transfer across various languages. For future endeavors, efforts could focus on translating the training data to enhance language variety, accumulating a wider range of multi-class classification tasks, or amalgamating several related binary classification tasks to form a more complex multi-class classification challenge.
